Evidence for the Typhon Stellar Stream as the Remnant of a Recently-disrupted Dwarf Galaxy

In the hierarchical model of galaxy formation, the Milky Way's stellar halo assembles through the successive accretion of dwarf galaxies. While many resulting substructures have been identified, the origin of the recently discovered Typhon stellar stream remains ambiguous, as dynamical data alone are insufficient to distinguish between a globular cluster and a dwarf galaxy progenitor. To resolve this, we combine astrometry from Gaia with spectroscopic data from available surveys to comprehensively analyze the stream's chemical and dynamical properties. We identify 107 candidate members, significantly expanding the known sample. Three of these candidates lie beyond $55\,\mathrm{kpc}$, with the farthest at $67\,\mathrm{kpc}$, lending further support to Typhon's inferred large apocentric distance. Our analysis yields a mean metallicity of $\rm[Fe/H]=-1.42\pm0.07$ and a metallicity dispersion of $\sigma_{\text{[Fe/H]}} = 0.26^{+0.06}_{-0.05}$ dex. This metallicity dispersion supports a dwarf-galaxy origin for the Typhon stream. Typhon's high orbital energy is consistent with a relatively recent accretion of a fully disrupted dwarf galaxy with a stellar mass in the range of $10^6 M_{\odot} < M_\star \lesssim 10^7 M_{\odot}$. Furthermore, Typhon is the only major dwarf-galaxy stellar stream in the Milky Way's halo to exhibit such an extreme orbital eccentricity of $e \gtrsim 0.85$. We conjecture that dwarf-galaxy streams from high-eccentricity mergers are fully dissolved much more rapidly than those on circular orbits, in line with Typhon's proposed recent accretion. Additional dwarf-galaxy stellar streams on high-eccentricity orbits should be discoverable with next-generation photometric surveys as well as future releases from the Gaia space mission.

==> EMPstars.tex <==
\begin{tabular}{ccccccccccccccccccccccc}
\hline
  \multicolumn{1}{|c|}{RA} &
  \multicolumn{1}{c|}{DEC} &
  \multicolumn{1}{c|}{fehs\_loggm08} &
  \multicolumn{1}{c|}{fehs\_errs\_08} &
  \multicolumn{1}{c|}{feh\_t23} &
  \multicolumn{1}{c|}{e\_feh\_t23} &
  \multicolumn{1}{c|}{feh\_h19} &
  \multicolumn{1}{c|}{e\_feh\_h19} &
  \multicolumn{1}{c|}{feh\_s15} &
  \multicolumn{1}{c|}{feh\_w23} &
  \multicolumn{1}{c|}{e\_feh\_w23} &
  \multicolumn{1}{c|}{X.M.H.\_ap} &
  \multicolumn{1}{c|}{e\_.M.H.\_ap} &
  \multicolumn{1}{c|}{X.Fe.H.\_ap} &
  \multicolumn{1}{c|}{e\_.Fe.H.\_ap} &
  \multicolumn{1}{c|}{feh\_c18} &
  \multicolumn{1}{c|}{e\_feh\_c18} &
  \multicolumn{1}{c|}{feh\_k09} &
  \multicolumn{1}{c|}{e\_feh\_k09} &
  \multicolumn{1}{c|}{feh\_r20} &
  \multicolumn{1}{c|}{e\_feh\_r20} &
  \multicolumn{1}{c|}{feh\_r22} &
  \multicolumn{1}{c|}{e\_feh\_r22} \\
\hline
  01:00:00.50 & -33:49:35.6 & -3.07 & 0.17 & -2.45 & 0.042 & -2.35 & 0.20 &  &  &  & -2.33 & 0.04 & -2.24 & 0.03 &  &  &  &  & -2.27 & 0.27 & -2.35 & 0.20\\
  01:00:47.84 & -33:41:03.2 & -3.35 & 0.2 &  &  &  &  & -3.68 &  &  &  &  &  &  & -3.63 & 0.21 & -3.8 & 0.28 &  &  & -3.87 & 0.23\\
  00:59:23.05 & -34:09:39.1 & -3.09 & 0.17 &  &  &  &  &  &  &  & -2.3 & 0.09 & -2.05 & 0.04 &  &  &  &  &  &  &  & \\
  01:00:05.02 & -34:01:16.6 & -3.36 & 0.2 & -3.17 & 0.07 &  &  & -3.31 & -2.78 & 0.14 &  &  &  &  &  &  &  &  & -3.13 & 0.2 &  & \\
  01:00:01.15 & -33:59:21.4 & -3.85 & 0.24 & -3.89 & 0.2 &  &  & -4.05 & -2.9 & 0.463 &  &  &  &  & -3.77 & 0.2 &  &  & -4.18 & 0.45 &  & \\
  00:57:11.39 & -34:00:11.3 & -3.08 & 0.3 & -2.69 & 0.12 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:57:44.16 & -34:01:14.3 & -3.15 & 0.17 & -3.33 & 0.09 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:59:25.64 & -33:58:21.5 & -3.05 & 0.16 & -2.66 & 0.06 &  &  &  & -2.91 & 0.38 & -1.88 & 0.04 & -1.78 & 0.025 & -3.1 & 0.16 &  &  &  &  &  & \\
  01:00:12.65 & -33:53:09.4 & -3.0 & 0.18 & -3.02 & 0.07 &  &  &  & -2.74 & 0.11 &  &  &  &  &  &  &  &  &  &  &  & \\
  00:58:05.52 & -33:55:16.4 & -3.12 & 0.17 & -3.06 & 0.05 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:55:29.88 & -33:46:05.9 & -3.01 & 0.2 & -2.74 & 0.17 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:57:10.22 & -33:28:35.8 & -3.86 & 0.34 & -3.62 & 0.13 &  &  &  &  &  &  &  &  &  &  &  &  &  & -3.91 & 0.24 &  & \\
  01:01:41.82 & -34:01:35.3 & -3.01 & 0.21 & -2.4 & 0.24 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  01:03:11.87 & -33:50:57.5 & -3.018 & 0.2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  01:01:30.84 & -33:57:30.1 & -3.01 & 0.17 & -2.53 & 0.05 &  &  &  &  &  &  &  & -2.38 & 0.03 &  &  &  &  &  &  &  & \\
  01:01:29.04 & -33:47:55.2 & -3.06 & 0.38 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  01:01:05.84 & -33:48:42.4 & -3.06 & 0.47 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  01:01:47.48 & -33:47:27.6 & -3.05 & 0.18 & -3.19 & 0.14 &  &  &  &  &  &  &  &  &  & -3.15 & 0.25 &  &  &  &  &  & \\
  01:00:48.69 & -33:35:48.1 & -3.03 & 0.36 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  01:00:00.41 & -33:29:15.5 & -3.09 & 0.19 & -3.53 & 0.38 &  &  & -3.53 &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:59:25.74 & -33:28:29.9 & -3.38 & 0.49 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
  00:58:50.64 & -32:54:04.7 & -3.13 & 0.23 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & \\
\hline\end{tabular}

==> notes_metalrich.tex <==

\section{Notes about [Fe/H] $> -1$ dex}
\label{rich}

\textbf{More ideas than actual text for this section} \\
We found that richer (redder) stars are more affected by the models used. Refining the grid, adding more models with [Fe/H] $> -1$, improved the metallicity estimated for a significant amount of stars in that region of the colour-colour diagram. However, we still observe some rich stars.

That is unexpected, since photometric metallicities tend to be worse in the metal-poor end ([Fe/H] $< -3$). Indeed, for stars with [Fe/H] $\lessapprox -1.5$, the uncertainty tends to be larger for lower values. The same behaviour is mirrored for the metal-rich end: the higher the metallicity, the higher the uncertainty. Furthermore, it's possible to distinguish two sequence in the metal-rich end (two because the number of star suddenly drop), where the richer corresponds to the group of stars that stands out on the MDF.

This metal-rich population is found mainly on the inner region of Scl, has low proper motions and tends to have $g > 20$, but there are some brighter stars. They are not particularly concentrated on the red clump. 

Even though our metallicities are worse compared to T23 in this regime, they also classify some metal-rich stars as Scl members. [C/Fe] from R22 points to abundances mostly between -0.2 and 0. Three stars have [Ba/Fe] $> 0$. 
Two stars are actually EMPs by C18, but no [C/Fe] is presented.

With the available data, we cannot affirm that this group is (in part or entirely) Milky Way contamination. Perhaps, part can be contamination, and another part are true members.  

Activity?

%% Fu23
% Possíveis problemas com o filtro CaHK afetam as estrelas mais pobres, não as mais ricas
% Qual a chance de ser contaminação na amostra?




This metal-rich population is found mainly on the inner region of the Scl dSph and tends to have $g > 20$, with some brighter stars. There is no compelling evidence to conclude that this is Milky Way contamination. 


==> table.tex <==
\begin{table}[ht]
\caption{Comparison of MAGIC data with spectroscopic samples. For each work, the number of stars in common (N) and the median values using the spectroscopic ($\rm[Fe/H]_{spec}$) and photometric ($\rm[Fe/H]_{MAGIC}$) estimates are presented. The median values of $\Delta\rm[Fe/H]$ are also provided ($\rm M_{\Delta[Fe/H]}$).} \label{tab:stat}
\centering
\begin{tabular}{lcccc}
\hline
  \multicolumn{1}{c}{Work} &
  \multicolumn{1}{c}{N} &
  \multicolumn{1}{c}{$\rm[Fe/H]_{spec}$} &
  \multicolumn{1}{c}{$\rm[Fe/H]_{MAGIC}$} & 
  \multicolumn{1}{c}{$\rm M_{\Delta[Fe/H]}$} \\
\hline \hline
  Tolstoy et al. (2023) & 1148 & -1.82 & -1.84 & -0.05 \\
  Walker et al. (2023) & 194 & -1.59 & -1.77 & -0.21 \\
  de los Reyes et al. (2022) -- [Fe/H] & 366 & -1.66 & -1.57 & 0.04 \\
  de los Reyes et al. (2022) -- [Ca/H] & 350 & -1.50 & -1.57 & -0.16 \\
  Reichert et al. (2020) & 77 & -1.56 & -1.79 & -0.21 \\
  Hill et al. (2019) & 76 & -1.57 & -1.74 & -0.17 \\
  Chiti et al. (2018) & 64 & -2.84 & -2.35 & 0.38 \\
  Kirby et al. (2009) & 328 & -1.58 & -1.55 & 0.04 \\
  APOGEE DR17 \citep{Abdurrouf2022_apogee} & 147 & -1.69 & -1.97 & -0.24 \\
\hline \hline 
\end{tabular}
\end{table}



==> table_stats.tex <==
\begin{table}[ht]
\caption{Summary of statistics for the MAGIC MDF (Figure \ref{fig:mdf}), including mean, median, standard deviation (SD), median absolute deviation (MAD), skewness, kurtosis, and quantiles (25th and 75th). Mean and median values with their respective deviation for the normalized difference (ND) histograms (Figure \ref{fig:norm_hist}) are listed here. The metallicity gradients estimated by single and segmented fits (SF) are also presented.} \label{main_tab}
\centering
\begin{tabular}{lc}
\hline
  \multicolumn{2}{c}{MAGIC MDF} \\
 % \multicolumn{1}{c}{N} &
 % \multicolumn{1}{c}{$\Delta\rm[Fe/H]$} \\
\hline \hline
  Median $\pm$ MAD & $-1.65 \pm 0.42$ \\ 
  Mean $\pm$ SD & $-1.67 \pm 0.46$ \\
  Skewness & 0.03 \\
  Kurtosis & 3.98 \\
  25th / 75th quantiles & $-1.97$ / $-1.39$ \\
  \hline
  \multicolumn{2}{c}{ND: Tolstoy et al. -- $\frac{\rm [Fe/H]_{MAGIC} - [Fe/H]_{T23} - C}{\sqrt{\sigma^2_{\rm T23} + \sigma_{\rm MAGIC}^2}}$} \\[0.2cm]
  \hline \hline
  Median $\pm$ MAD & $0.0 \pm 1.1$ \\
  Mean $\pm$ SD & $0.0 \pm 1.3$ \\
  \hline
  \multicolumn{2}{c}{ND: de los Reyes et al. -- $\frac{\rm [Fe/H]_{MAGIC} - [Fe/H]_{R22} - C}{\sqrt{\sigma^2_{\rm R22} + \sigma_{\rm MAGIC}^2}} $} \\[0.2cm]
  \hline \hline
  Median $\pm$ MAD & $0.0 \pm 1.1$ \\
  Mean $\pm$ SD & $0.1 \pm 1.2$ \\
  \hline
  \multicolumn{2}{c}{Metallicity gradients } \\
  \hline \hline
  \multirow{3}{4cm}{Single linear fit} & $-1.00 \pm 0.03 \rm \ dex \, deg^{-1}$ \\
    & $-0.19 \pm 0.01 \rm \ dex \, r_h^{-1}$ \\
    & $-0.68 \pm 0.18 \rm \ dex \, kpc^{-1}$ \\[0.15cm]
  \multirow{3}{4cm}{SF: until $1.06 \ \rm r_h$} & $-3.26 \pm 0.18 \rm \ dex \, deg^{-1}$ \\
   & $-0.61 \pm 0.03 \rm \ dex \, r_h^{-1}$ \\
    & $-2.22 \pm 0.60 \rm \ dex \, kpc^{-1}$ \\[0.15cm]
  \multirow{3}{4cm}{SF: beyond $1.06 \ \rm r_h$} & $-0.55 \pm 0.26 \rm \ dex \, deg^{-1}$ \\
   & $-0.10 \pm 0.05 \rm \ dex \, r_h^{-1}$ \\
    & $-0.38 \pm 0.20 \rm \ dex \, kpc^{-1}$ \\
\hline \hline 
\end{tabular}
\end{table}


